A high-order finite volume method for Maxwell's equations in heterogeneous and time-varying media

We develop a finite volume method for Maxwell's equations in materials whose electromagnetic properties vary in space and time. We investigate both conservative and non-conservative numerical formulations. High-order methods accurately resolve fine structures that develop due to the varying material properties. Numerical examples demonstrate the effectiveness of the proposed method in handling temporal variation and its efficiency relative to traditional 2nd-order FDTD.

==> fig-1.tex <==
% -------------- figure 1 tikz --------------
% Define block styles
\tikzstyle{decision} = [diamond, draw, fill=blue!20, text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=blue!20, text width=8em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm, minimum height=2em]    
%\begin{tikzpicture}[node distance = 2cm, auto]
    % Place nodes
    \node [block] (init) {Set $\bar\eta$ and $\F$ at $t_{n}$};
%    \node [cloud, left of=init] (expert) {expert};
%    \node [cloud, right of=init] (system) {system};
    \node [block, below of=init] (identify) {calculate $Q_i^n$};
    \node [block, below of=identify] (evaluate) {evaluate flux difference};
    \node [decision, left of=evaluate, node distance=4cm] (update) {advance $t_{n+1}$, update $Q_i^{n+1}$};
    \node [block, below of=evaluate] (decide) {solve Riemann problem};
    \node [block, below of=decide, node distance=2cm] (stop) {stop};
    % Draw edges
     \path [line] (init) -- (identify);
    \path [line] (identify) -- (evaluate);
    \path [line] (evaluate) -- (decide);
    \path [line] (decide) -| node [near start] {~} (update);
    \path [line] (update) |- (init);
    \path [line] (decide) -- node {~}(stop);
%    \path [line,dashed] (expert) -- (init);
%    \path [line,dashed] (system) -- (init);
 %   \path [line,dashed] (system) |- (evaluate);
%\end{tikzpicture}


